Lying Aversion and Vague Communication: An Experimental Study

An agent may strategically employ a vague message to mislead an audience's belief about the state of the world, but this may cause the agent to feel guilt or negatively impact how the audience perceives the agent. Using a novel experimental design that allows participants to be vague while at the same time isolating the internal cost of lying from the social identity cost of appearing dishonest, we explore the extent to which these two types of lying costs affect communication. We find that participants exploit vagueness to be consistent with the truth, while at the same time leveraging the imprecision to their own benefit. More participants use vague messages in treatments where concern with social identity is relevant. In addition, we find that social identity concerns substantially affect the length and patterns of vague messages used across the treatments.

==> lying_main-pratenddefaultcategory.tex <==


\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}\hfill \begin {enumerate}[{Case }1.] \item Anonymous environment: as shown in Proposition \ref {pr:A-UR_report}, all truth-tellers use the optimal vague message. \item Non-anonymous environment: suppose there exists an equilibrium where no agent uses a vague message. Let $\rho (j)=0$ for all $j \in M^{\Omega }_{V}$. Given that all messages used with positive probability are precise, we know all precise messages are used with positive probability in this equilibrium. We use Lemma \ref {lm:NA-R_lie} and \ref {lm:NA-R_no-under} to argue that there exists a positive probability that agents lie upward. Let $l^{*}$ be the threshold defined in Lemma \ref {lm:NA-R_threshold}. \par Let us first argue that there exists agents who observe $l^{*}-1$ and lie by reporting $l^{*}$. Suppose not. Then there must exist some $l > l^{*}$ such that \begin {align*} U(l^{*}-1, l, t)-U(l^{*}-1, l^{*}, t) = (l- l^{*}) + (c(l^{*}-1, l^{*}) - c(l^{*}-1, l)) + \gamma (\rho (l)- \rho (l^{*})) >0. \end {align*} Note that $c(l^{*}-1, l^{*}) - c(l^{*}-1, l) \leq 0$ because $l > l^{*}$ and $c$ is increasing in the distance between the two arguments. Also, $c(l^{*}-1, l^{*}) - c(l^{*}-1, l) \leq c(i, l^{*}) - c(i, l) \leq 0$ for all $i < l^{*}$ because of the triangular inequality assumption. This implies that for all agents whose true observation is below $l^{*}$ is better off by reporting $l$ instead of $l^{*}$. As no agent would lie by reporting $l^{*}$, this is a contradiction to the definition of threshold. \par Now consider the agent who observes $l^{*}-1$ and lies by reporting $l^{*}$. The agent receives the utility of $$ U(l^{*}-1, l^{*}, t) = l^{*} - (t + c(l^{*}-1, l^{*})) + \gamma \rho (l^{*}). $$ However, if the agent reports $\{l^{*}-1, l^{*}+1\}$ instead, the agent receives $$ U(l^{*}-1, \{l^{*}-1, l^{*}+1\}, t) = l^{*}. $$ That is, the agent is better off by reporting $\{l^{*}-1, l^{*}+1\}$ when $$ t > \gamma \rho (l^{*}) -c(l^{*}-1, l^{*}), $$ which happens with a positive probability. Furthermore, the above analysis is valid for all $\rho (\{l^{*}-1, l^{*}+1\}) \geq 0$. This is a contradiction to the assumption of an equilibrium with no vague messages. Therefore, there exists a positive probability that agents use a vague message in any equilibrium in the NA-UR environment. \end {enumerate} \par \end{proof}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}\begin {enumerate} \item By the definition of the OVM, it is the message that maximizes the utility of an agent who observes state $i$ conditional on including the true state $i$ in their message. If $\argmax _{J: i \in J} U(i, J, t)$ is a singleton set, we are done. If not, the agent may use another message in $\argmax _{J: i \in J} U(i, J, t)$, but the expected earning is still the same. \item Suppose an agent reports a message $J$ with $\min J < i$. Then the message $J \cup \{i\} \setminus \{ \min J \}$ strictly dominates $J$. \item Suppose an agent truthfully reports $\{i\}$. If $i = N$, we are done. If not, the message is strictly dominated by $OVM_i$. \end {enumerate}\end{proof}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}Let $j>i$ be a part of an equilibrium strategy for an $(i,t)$-agent in the NA-R environment: \begin {equation*} U(i,j,t)=j-[t+c(i,j)]+\gamma \rho (j) \geq U(i, j^{\prime }, t) \quad \forall j^{\prime } \in M^{\Omega }_P. \end {equation*} \par We can infer that \begin {equation*} j-[t+c(i,j)]+\gamma \rho (j) \geq i + \gamma \rho (i), \end {equation*} or \begin {equation*} (j-i) - [t + c(i,j)] \geq \gamma (\rho (i) - \rho (j)). \end {equation*} \par As no agent underreports in the A-R environment, it suffices to show that this agent does not tells the truth in the A-R. Suppose not. \begin {equation*} U_A (i, i, t) = i > U_A (i, j, t) = j - [t + c(i,j)] . \end {equation*} \par This implies $\rho (i) < \rho (j)$, meaning the agent lied in the NA-R both because there were a monetary gain and a social identity gain. \begin {align*} (j-i) + [c(i^{\prime },i) - c(i^{\prime },j)] + \gamma (\rho (j) - \rho (i)) & \geq c(i^{\prime },i) - c(i^{\prime },j) + t + c(i,j) >0 \end {align*} because of the triangular inequality assumption: $c(i, i^{\prime }) + c(i^{\prime }, j) \geq c(i,j)$. As the choice of this agent is arbitrary, this is the case for all agents who do not observe $i$ never lies by reporting $i$; in turn, this implies $\rho (i)=1$, a contradiction. Therefore, the agent must lie in the A-R if the agent sees the same observation $i$.\end{proof}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}WTS $P(\text {lie}_{NA-R}) < P(\text {lie}_{A-R})$. \par We argue by the law of total probability: \begin {align*} P(\text {lie}_{NA-R}) & = \sum ^{N}_{i=1} P(\text {observe $i$}) P(\text {lie}_{NA-R} | \text {observe $i$}); \\ P(\text {lie}_{A-R}) & = \sum ^{N}_{i=1} P(\text {observe $i$}) P(\text {lie}_{A-R} | \text {observe $i$}). \end {align*} Because the probability of observing some $i$ is uniform in both environments, it suffices to show that the conditional probability of lying in A-R is greater than or equal to that in NA-R for all true observation $i$. \par We learned that there exists some threshold $1<l^{*}<N$ in Lemma \ref {lm:NA-R_threshold}. Thus, conditional on that an agent observing $i \geq l^{*}$, we have the conditional probability of the agent reporting a lie as $$ P(\text {lie}_{NA-R} | \text {observe $i$}) = 0; $$ for all intrinsic aversion type $t$, while $$ P(\text {lie}_{A-R} | \text {observe $i$}) >0 $$ because of the positive probability that the agent has the type $t$ small enough to report a lie. \par Now consider the case of $i < l^{*}$. Let $T_i$ be a subset of $\mathbb {R}$ such that \begin {align*} P(\text {lie}_{NA-R} | \text {observe $i$}, t \in T_i) > 0; \\ P(\text {lie}_{NA-R} | \text {observe $i$}, t \not \in T_i) = 0. \end {align*} \par By Lemma \ref {lm:NA-R_then-A-R}, $P(\text {lie}_{A-R} | \text {observe $i$}, t \in T_i) = 1$; and $P(\text {lie}_{A-R} | \text {observe $i$}, t \not \in T_i) \geq 0$. Thus, regardless of $P(t \in T_i)$, we have $$ P(\text {lie}_{NA-R} | \text {observe $i$}) \leq P(\text {lie}_{A-R} | \text {observe $i$}) $$ for all $i < l^{*}$. Therefore, $P(\text {lie}_{NA-R}) < P(\text {lie}_{A-R})$. \par Also, because the monetary payment is a monotone mapping of the reports under the restricted communication, and because any lying takes the form of reporting upward, agents would earn more monetary payoff on average as the probability of lying is greater in the A-R.\end{proof}

